Inclusive Jet Cross-section measurement at CDF

Results on inclusive jet production in proton-antiproton collisions at sqrt(s) =1.96 TeV based on 1 fb-1 of CDF Run II data are presented. Measurements are preformed using the k_T algorithm in a wide range of jet transverse momentum and jet rapidity. The measured cross sections are compared to next-to-leading order perturbative QCD calculations.

==> abstract_moriond.tex <==
Results on inclusive jet production in proton-antiproton collisions at 
sqrt(s) =1.96 TeV based on $1 fb-1 of CDF  Run II data are presented. 
Measurements are preformed using the kT algorithm in a wide range of jet transverse momentum 
and jet rapidity. The measured cross sections are compared to next-to-leading order perturbative QCD calculations.

